Query-Guided Networks for Few-shot Fine-grained Classification and Person Search

Few-shot fine-grained classification and person search appear as distinct tasks and literature has treated them separately. But a closer look unveils important similarities: both tasks target categories that can only be discriminated by specific object details; and the relevant models should generalize to new categories, not seen during training. We propose a novel unified Query-Guided Network (QGN) applicable to both tasks. QGN consists of a Query-guided Siamese-Squeeze-and-Excitation subnetwork which re-weights both the query and gallery features across all network layers, a Query-guided Region Proposal subnetwork for query-specific localisation, and a Query-guided Similarity subnetwork for metric learning. QGN improves on a few recent few-shot fine-grained datasets, outperforming other techniques on CUB by a large margin. QGN also performs competitively on the person search CUHK-SYSU and PRW datasets, where we perform in-depth analysis.

==> tables/prw/ablation.tex <==
\begin{table}
\setlength{\tabcolsep}{4.5pt}
\renewcommand{\arraystretch}{0.8}
\caption{Person search accuracy on PRW dataset, using different design choices. For PRW the whole test set is used. Second column gives the image size. $Pool(n)$ refers to ROI pool operation and $Align(n)$ refers to ROI align operation with output size $n\times n$. gCat refers to the concatenation of globally pooled ROI align feature with ClsIdenNet output feature (Fig.~\ref{fig:network}).
\vspace{-0.1cm}
} 

\begin{center}
\begin{tabular}{ccccccccc}
\hline
& & & &  &\multicolumn{2}{c}{\textbf{CUHK}}   &\multicolumn{2}{c}{\textbf{PRW}} \\
\cmidrule(l){6-7} \cmidrule(l){8-9}
 \bf{Model} & \bf{imSize} & \bf{ROI}  & \bf{bSize} & \bf{gCat}  & \bf{mAP}  & \bf{top-1}& \bf{mAP}  & \bf{top-1}\\
\hline
\hline
OIM & 600 & $Pool(7)$ &  1 & &77.2 & 77.6 & 29.2&  65.0\\
OIM & 600 & $Pool(14)$ &  1 &  & 80.8 & 80.9 & 32.8 & 71.3\\
OIM & 600 & $Align(14)$ & 1 & & 81.2 & 81.7 & 33.6 & 71.4\\
OIM & 900 & $Align(14)$ & 1& & 83.9 & 84.2 & 36.9 & 75.7\\
OIM & 900 & $Align(14)$ & 2& &86.1  & 87.8 & 38.7 & 78.4\\
{OIM} & {900} & {$Align(14)$} & {2}& {\checkmark} & {88.6}  &  {88.8} & {40.4} & {79.2}\\
\textbf{QGN} & 900 & $Align(14)$  & 2 & \checkmark  &\textbf{91.5}  &  \textbf{92.1} & \textbf{42.9} & \textbf{80.9} \\
\hline
 

\end{tabular}
\end{center}

%\vspace{-0.5cm}
\label{tab:cuhk_analysis}
\end{table}



